Is Your Video Language Model a Reliable Judge?

As video language models (VLMs) gain more applications in various scenarios, the need for robust and scalable evaluation of their performance becomes increasingly critical. The traditional human expert-based evaluation of VLMs has limitations in consistency and scalability, which sparked interest in automatic methods such as employing VLMs to evaluate VLMs. However, the reliability of VLMs as judges remains underexplored. Existing methods often rely on a single VLM as the evaluator. However, this approach can be unreliable or biased because such a model may lack the ability to fully understand the content and may have inherent biases, ultimately compromising evaluation reliability. A remedy is to apply the principle of collective thoughts, aggregating evaluations from multiple VLMs to enhance reliability. This study investigates the efficacy of such approaches, particularly when the pool of judges includes both reliable and unreliable models. Our findings reveal that incorporating collective judgments from such a mixed pool does not necessarily improve the accuracy of the final evaluation. The inclusion of less reliable judges can introduce noise, undermining the overall reliability of the outcomes. To explore the factors that impact evaluation reliability, we fine-tune an underperforming VLM judge, Video-LLaVA, and observe that improved understanding ability alone is insufficient to make VLM judges more reliable. These findings stress the limitations of collective thought approaches and highlight the need for more advanced methods that can account for the reliability of individual models. Our study promotes the development of more reliable evaluation methods for VLMs

==> table/agreement_avereage.tex <==
\begin{table}[htbp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|ccccccccccc}
    \hline
     & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
    \cline{2-12}
    \textbf{Judge} & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
    \hline
    \textbf{Video-LLaVA} & 1.35 & 0.52 & 2.15 & 2.81 & 1.00 & -1.83 & -1.38 & 0.47 & 0.68 & 0.23 & 0.37 \\
    \textbf{LLaMA-VID} & 3.70 & 1.66 & 1.32 & 3.08 & 1.39 & -4.15 & -4.04 & 2.00 & 2.99 & 0.23 & 0.37 \\
    \textbf{InternVL2} & 10.69 & 13.47 & 12.08 & 16.71 & 9.52 & 2.18 & 3.10 & 3.21 & 9.33 & 7.50 & 6.10 \\
  \textbf{GPT-4o mini} & 14.50 & 21.43 & 21.18 & 22.28 & 17.53 & -1.62 & -1.09 & 1.94 & 6.78 & 12.11 & 7.27
    \\
    \textbf{GPT-4o} & 33.11 & 54.41 & 60.38 & 55.18 & 44.24 & 35.09 & 23.09 & 45.30 & 34.40 & 32.23 & 30.65 \\
    \hline
    \end{tabular}
    \caption{Agreement scores(\%) across various visual dimensions between VLMs and Agent-Debate}
    \label{tab:agreement_avereage}
\end{table}


==> table/baseline.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccccccccccc}
\hline
\textbf{Candidate} & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
\cline{2-12}
 & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
\hline
LLaMA-VID & 33.66 & 54.43 & 60.79 & 43.13 & 43.08 & 16.74 & 6.99 & 31.50 & 26.41 & 32.23 & 30.87 \\
GPT-4o mini & \textbf{42.58} & 39.71 & 42.07 & 50.45 & 37.04 & 35.67 & 21.15 & \textbf{50.29} & 36.87 & 24.59 & 25.22 \\
Video-ChatGPT & 41.44 & \textbf{61.71} & \textbf{69.39} & 58.41 & \textbf{56.87} & \textbf{61.53} & 29.74 & 46.53 & 36.29 & 31.45 & \textbf{35.47} \\
mPLUG-Owl-Video & 22.73 & 57.36 & 63.28 & \textbf{64.64} & 41.08 & 34.49 & 23.56 & 49.32 & \textbf{38.89} & 35.09 & 29.93 \\
Video-LLaVA & 25.16 & 58.85 & 66.35 & 59.28 & 43.14 & 27.01 & \textbf{34.00} & 48.85 & 33.57 & \textbf{37.80} & 31.75 \\
\hline
\textit{Average} & 33.11 & 54.41 & 60.38 & 55.18 & 44.24 & 35.09 & 23.09 & 45.30 & 34.40 & 32.23 & 30.65 \\
\hline
\end{tabular}
\caption{Agreement scores across various CVRR (Computer Vision and Robotics Research) dimensions for judge \texttt{interpolated-judge}}
\label{tab:cvrr_scores}
\end{table}


==> table/gpt_3.5.tex <==

% \begin{table}[!t]
%     \caption{\small Average performance of video language models on various visual dimensions.}
%     \small \centering
%  \setlength{\tabcolsep}{6pt}
%  \tabstyle{2pt}
%     \scalebox{0.76}[0.76]{
% \begin{tabular}{l | cccccccccccc}
% \toprule
% {Model}  & 
%  \parbox{1.5cm}{\centering Continuity} &
%  \parbox{1.5cm}{\centering Fine Action}  & 
%  \parbox{1.5cm}{\centering Social Context}  & 
%  \parbox{1.5cm}{\centering Visual Context}  &
%  \parbox{1.5cm}{\centering Multiple Actions} &
%  \parbox{1.5cm}{\centering Existent Actions} &
%  \parbox{1.5cm}{\centering Non-existent Actions} &
%  \parbox{1.5cm}{\centering Partial Actions} &
%  \parbox{1.5cm}{\centering Time Order} &
%  \parbox{1.5cm}{\centering Emotional Context} &
%  \parbox{1.5cm}{\centering Anomalous Activities} &
%  \parbox{1.5cm}{\centering Average}
% \\  \midrule

% {LLaMA\_vid}    & 0.11870 & 0.29933 & 0.24142 & 0.28476 & 0.18579 & 0.12537 & 0.04584 & 0.10538 & 0.03510 & 0.22730 & 0.19725 & 0.17540 \\ 
% {gpt4v}         & 0.12582 & 0.02740 & 0.04647 & 0.12050 & 0.09361 & -0.18426 & -0.29911 & -0.05314 & 0.01585 & -0.13238 & -0.20937 & 0.03157 \\
% {video\_chatgpt} & 0.08487 & 0.21632 & 0.21888 & 0.13776 & 0.12956 & -0.08611 & -0.15861 & -0.05051 & 0.08816 & 0.08703 & 0.10261 & 0.04597 \\
% {mplug\_owl\_Video} & 0.12924 & 0.28814 & 0.23792 & 0.25973 & 0.14699 & 0.06419 & 0.04425 & 0.02626 & 0.19762 & 0.22465 & 0.09992 & 0.17540 \\
% {video\_LLaVA}   & 0.12803 & 0.32516 & 0.13233 & 0.05697 & 0.20504 & 0.00480 & -0.07064 & -0.02331 & 0.11362 & 0.18544 & 0.14526 & 0.11733 \\ 
% {average}       & 0.11733 & 0.23127 & 0.17540 & 0.17194 & 0.15220 & -0.01520 & -0.08765 & 0.00094 & 0.09007 & 0.11841 & 0.06713 & 0.06713 \\

% \bottomrule
% \end{tabular}
% }
%     \label{tab:average_performance_cvrr_short_names}
% \end{table}




% =========


\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccccccccccc}
\hline
\textbf{Candidate} & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
\cline{2-12}
\textbf{\& Judge} & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
\hline
\multicolumn{12}{l}{\textbf{LLaMA-VID}} \\
Video-LLaVA & \textbf{3.95} & \textbf{3.98} & \textbf{4.00} & \textbf{4.00} & \textbf{3.98} & \textbf{3.96} & \textbf{3.96} & \textbf{3.99} & \textbf{4.00} & \textbf{4.00} & \textbf{3.98} \\
LLaMA-VID & 3.81 & 3.83 & 3.92 & 3.90 & 3.76 & 3.94 & 3.81 & 3.85 & 3.84 & 3.85 & 3.76 \\
GPT-4o mini & 2.51 & 3.07 & 2.50 & 2.64 & 2.60 & 2.53 & 2.27 & 2.93 & 3.18 & 2.74 & 2.33 \\
InternVL2 & 3.12 & 3.63 & 3.31 & 3.36 & 3.55 & 3.46 & 3.12 & 3.63 & 3.56 & 3.34 & 3.09 \\
GPT-3.5 & 2.31 & 2.30 & 1.85 & 2.05 & 2.01 & 1.06 & 1.16 & 1.73 & 2.24 & 1.90 & 1.95 \\
\hline
\multicolumn{12}{l}{\textbf{GPT-4o mini}} \\
Video-LLaVA & \textbf{3.86} & 3.88 & 3.85 & \textbf{3.86} & \textbf{3.73} & 3.57 & 3.69 & \textbf{3.84} & 3.91 & \textbf{3.87} & \textbf{3.93} \\
LLaMA-VID & 3.71 & 3.79 & 3.73 & 3.75 & 3.54 & 3.46 & 3.43 & 3.67 & 3.82 & 3.67 & 3.79 \\
GPT-4o mini & 2.81 & 3.43 & 3.29 & 3.20 & 2.93 & 2.83 & 2.63 & 3.20 & 3.55 & 3.15 & 3.12 \\
InternVL2 & 3.14 & 3.59 & 3.57 & 3.57 & 3.39 & 3.33 & 3.20 & 3.43 & 3.60 & 3.47 & 3.64 \\
GPT-3.5 & 3.41 & \textbf{3.90} & \textbf{3.95} & 3.73 & 3.21 & \textbf{3.80} & \textbf{3.74} & 3.73 & \textbf{3.93} & 3.20 & 3.49 \\
\hline
\multicolumn{12}{l}{\textbf{Video-ChatGPT}} \\
Video-LLaVA & \textbf{3.99} & \textbf{4.00} & \textbf{3.99} & \textbf{4.00} & \textbf{4.00} & \textbf{3.98} & \textbf{4.00} & \textbf{4.00} & \textbf{3.99} & \textbf{3.99} & \textbf{3.99} \\
LLaMA-VID & 3.83 & 3.87 & 3.93 & 3.92 & 3.82 & 3.90 & 3.83 & 3.82 & 3.80 & 3.87 & 3.83 \\
GPT-4o mini & 2.17 & 2.86 & 2.52 & 2.50 & 2.43 & 2.37 & 2.40 & 2.62 & 2.92 & 2.70 & 2.29 \\
InternVL2 & 3.02 & 3.42 & 3.25 & 3.21 & 3.37 & 3.33 & 3.03 & 3.41 & 3.53 & 3.21 & 3.07 \\
GPT-3.5 & 2.66 & 2.34 & 2.60 & 2.53 & 2.48 & 1.75 & 1.62 & 2.17 & 2.34 & 2.05 & 1.96 \\
\hline
\multicolumn{12}{l}{\textbf{mPLUG-Owl-Video}} \\
Video-LLaVA & \textbf{4.00} & \textbf{3.99} & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} & 4.00 & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} \\
LLaMA-VID & 3.90 & 3.93 & 3.95 & 3.94 & 3.86 & \textbf{4.03} & 3.94 & 3.92 & 3.91 & 3.95 & 3.97 \\
GPT-4o mini & 2.44 & 3.03 & 2.64 & 2.84 & 2.46 & 2.60 & 2.40 & 2.77 & 3.15 & 2.82 & 2.43 \\
InternVL2 & 3.22 & 3.64 & 3.44 & 3.49 & 3.49 & 3.53 & 3.16 & 3.54 & 3.70 & 3.44 & 3.46 \\
GPT-3.5 & 2.27 & 2.46 & 2.35 & 2.34 & 2.02 & 1.11 & 1.10 & 2.00 & 2.33 & 1.95 & 1.99 \\
\hline
\multicolumn{12}{l}{\textbf{Video-LLaVA}} \\
Video-LLaVA & \textbf{3.98} & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} & \textbf{4.00} & \textbf{3.99} & \textbf{3.97} & \textbf{4.00} & \textbf{4.00} & \textbf{3.99} & \textbf{4.00} \\
LLaMA-VID & 3.87 & 3.84 & 3.91 & 3.95 & 3.78 & 3.97 & 3.83 & 3.82 & 3.84 & 3.86 & 3.85 \\
GPT-4o mini & 2.38 & 2.91 & 2.35 & 2.45 & 2.39 & 2.46 & 2.17 & 2.60 & 2.91 & 2.57 & 2.09 \\
InternVL2 & 3.28 & 3.65 & 3.39 & 3.36 & 3.43 & 3.38 & 3.17 & 3.67 & 3.59 & 3.29 & 3.10 \\
GPT-3.5 & 2.46 & 2.39 & 2.26 & 2.29 & 2.01 & 1.02 & 1.24 & 1.80 & 2.23 & 1.94 & 1.89 \\
\hline
\end{tabular}
\caption{Scores of candidate models given by judge models across various CVRR (Computer Vision and Robotics Research) dimensions}
\label{tab:cvrr_scores}
\end{table}


\paragraph{Contrasting Reviews from MLLM and LLM}
\leavevmode\\ 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figure/agreement.png}
%     \caption{Diagram illustrating the multi-stage evaluation process involving multiple initial reviews and a final comprehensive review by an advanced model.}
%     \label{fig:agreement}
% \end{figure}


\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccccccccccc}
\hline
\textbf{Judge} & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
\cline{2-12}
\textbf{\& Candidate} & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
\hline
\multicolumn{12}{l}{\textbf{Video-LLaVA}} \\
Video-LLaVA & \textbf{0.0029} & \textbf{0.0065} & 0.0000 & 0.0000 & 0.0000 & -0.0069 & -0.0133 & 0.0000 & 0.0000 & -0.0012 & 0.0000 \\
LLaMA-VID & -0.0059 & -0.0063 & 0.0000 & 0.0002 & -0.0020 & -0.0202 & -0.0182 & -0.0092 & 0.0000 & -0.0038 & -0.0042 \\
GPT-4o mini & \textbf{0.0368} & -0.0528 & \textbf{0.0969} & \textbf{0.1451} & -0.0242 & -0.1441 & -0.1513 & \textbf{0.0254} & \textbf{0.0271} & -0.0023 & -0.0063 \\
Video-ChatGPT & 0.0072 & 0.0008 & -0.0027 & 0.0000 & 0.0000 & -0.0186 & 0.0000 & -0.0051 & -0.0079 & -0.0036 & -0.0097 \\
mPLUG-Owl-Video & 0.0000 & 0.0044 & 0.0000 & 0.0000 & 0.0000 & \textbf{0.0000} & \textbf{0.0000} & 0.0000 & 0.0000 & -0.0013 & 0.0000 \\
\textit{Average} & 0.0082 & -0.0095 & 0.0188 & 0.0291 & -0.0052 & -0.0380 & -0.0366 & 0.0022 & 0.0038 & -0.0024 & -0.0040 \\
\hline
\multicolumn{12}{l}{\textbf{LLaMA-VID}} \\
LLaMA-VID & \textbf{0.0165} & -0.0110 & -0.0088 & -0.0173 & -0.0204 & \textbf{0.0018} & -0.0482 & -0.0127 & 0.0301 & -0.0021 & -0.0187 \\
Video-LLaVA & -0.0009 & \textbf{0.0056} & -0.0233 & -0.0012 & -0.0062 & -0.0180 & -0.0350 & -0.0007 & \textbf{0.0356} & -0.0102 & \textbf{0.0053} \\
GPT-4o mini & \textbf{0.0882} & \textbf{0.0068} & \textbf{0.0129} & \textbf{0.1245} & -0.0289 & -0.2003 & -0.2111 & \textbf{0.0049} & \textbf{0.0541} & -0.0214 & -0.0580 \\
Video-ChatGPT & 0.0470 & -0.0156 & -0.0011 & -0.0091 & \textbf{0.0428} & -0.0542 & -0.0331 & -0.0104 & -0.0013 & -0.0197 & -0.0266 \\
mPLUG-Owl-Video & 0.0067 & 0.0033 & -0.0277 & -0.0014 & -0.0143 & 0.0003 & -0.0039 & \textbf{0.0122} & 0.0211 & -0.0114 & -0.0015 \\
\textit{Average} & 0.0315 & -0.0022 & -0.0096 & 0.0191 & -0.0054 & -0.0541 & -0.0662 & -0.0013 & 0.0279 & -0.0130 & -0.0199 \\
\hline
\multicolumn{12}{l}{\textbf{GPT-4o mini}} \\
GPT-4o mini & 0.1214 & 0.0309 & 0.0419 & 0.1205 & 0.0924 & -0.1790 & -0.2933 & -0.0531 & -0.0051 & -0.1319 & -0.2058 \\
LLaMA-VID & 0.1144 & \textbf{0.3012} & \textbf{0.2532} & \textbf{0.3006} & 0.1758 & \textbf{0.1276} & -0.0042 & \textbf{0.0933} & 0.0574 & \textbf{0.2188} & \textbf{0.1933} \\
Video-LLaVA & 0.1173 & \textbf{0.3309} & 0.1284 & 0.0655 & \textbf{0.1922} & -0.0001 & -0.1056 & -0.0393 & \textbf{0.1143} & 0.1833 & 0.1117 \\
Video-ChatGPT & 0.0811 & 0.2120 & 0.2213 & 0.1644 & 0.1225 & -0.1410 & -0.1914 & -0.0460 & 0.0931 & 0.0863 & 0.1010 \\
mPLUG-Owl-Video & \textbf{0.1282} & 0.2733 & 0.2365 & 0.2730 & 0.1450 & 0.0601 & -0.0017 & 0.0231 & \textbf{0.2064} & 0.2137 & 0.0747 \\
\textit{Average} & 0.1125 & 0.2297 & 0.1763 & 0.1848 & 0.1456 & -0.0265 & -0.1192 & -0.0044 & 0.0932 & 0.1140 & 0.0550 \\
\hline
\multicolumn{12}{l}{\textbf{InternVL2}} \\
InternVL2 & 0.1208 & 0.1164 & 0.1073 & 0.1926 & 0.0962 & 0.0030 & -0.0108 & 0.0110 & 0.1203 & 0.0630 & 0.0335 \\
LLaMA-VID & 0.1249 & 0.0953 & 0.1101 & 0.1407 & 0.0520 & 0.0239 & \textbf{0.0019} & \textbf{0.0356} & 0.0643 & 0.0843 & \textbf{0.0354} \\
GPT-4o mini & \textbf{0.1309} & 0.0456 & 0.0627 & \textbf{0.2758} & \textbf{0.1296} & -0.0894 & -0.1101 & 0.0183 & \textbf{0.1712} & -0.0291 & -0.0435 \\
Video-LLaVA & 0.1277 & 0.1240 & \textbf{0.1396} & 0.1649 & 0.0714 & \textbf{0.0495} & \textbf{0.0490} & 0.0194 & 0.1328 & \textbf{0.1096} & \textbf{0.0758} \\
Video-ChatGPT & 0.0912 & \textbf{0.1777} & 0.0993 & \textbf{0.2160} & \textbf{0.1596} & -0.0187 & -0.0098 & -0.0234 & 0.1106 & 0.0478 & 0.0665 \\
mPLUG-Owl-Video & \textbf{0.1293} & \textbf{0.1393} & \textbf{0.1250} & 0.1655 & 0.0686 & 0.0494 & 0.0150 & 0.0051 & 0.1226 & \textbf{0.1023} & 0.0333 \\
\textit{Average} & 0.1208 & 0.1164 & 0.1073 & 0.1926 & 0.0962 & 0.0030 & -0.0108 & 0.0110 & 0.1203 & 0.0630 & 0.0335 \\
\hline
\end{tabular}
\caption{Agreement scores across various CVRR (Computer Vision and Robotics Research) dimensions}
\label{tab:cvrr_scores}
\end{table}

\paragraph{Naive ensemble method}

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccccccccccc}
\hline
\textbf{Candidate} & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
\cline{2-12}
 & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
\hline
LLaMA-VID & 0.1132 & \textbf{0.3012} & \textbf{0.2532} & 0.1289 & \textbf{0.1758} & \textbf{0.0239} & --- & \textbf{0.0356} & 0.0584 & \textbf{0.2188} & \textbf{0.1933} \\
GPT-4o mini & 0.1109 & 0.0309 & 0.0419 & \textbf{0.2775} & 0.0924 & -0.0894 & --- & 0.0183 & \textbf{0.1661} & -0.1319 & -0.2058 \\
Video-ChatGPT & 0.0983 & 0.2120 & 0.2213 & 0.1988 & 0.1225 & -0.0187 & --- & -0.0234 & 0.0930 & 0.0863 & 0.1010 \\
mPLUG-Owl-Video & 0.1280 & 0.2733 & 0.2365 & 0.1560 & 0.1450 & 0.0494 & --- & 0.0051 & 0.1183 & 0.2137 & 0.0747 \\
Video-LLaVA & \textbf{0.1362} & \textbf{0.3309} & 0.1284 & 0.1518 & \textbf{0.1922} & \textbf{0.0495} & --- & 0.0194 & 0.1170 & 0.1833 & 0.1117 \\
\hline
\textit{Average} & 0.1173 & 0.2297 & 0.1763 & 0.1826 & 0.1456 & 0.0030 & --- & 0.0110 & 0.1106 & 0.1140 & 0.0550 \\
\hline
\end{tabular}
\caption{Agreement scores across various CVRR (Computer Vision and Robotics Research) dimensions for judge \texttt{interpolated-judge}}
\label{tab:cvrr_scores}
\end{table}



\paragraph{Collective thoughts with all judge}

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccccccccccc}
\hline
\textbf{Judge} & \multicolumn{11}{c}{\textbf{visual dimensions}} \\
\cline{2-12}
\textbf{\& Candidate} & \rotatebox{70}{Cont. \& Obj.} & \rotatebox{70}{Fine Action} & \rotatebox{70}{Social Context} & \rotatebox{70}{Visual Context} & \rotatebox{70}{Multi Actions} & \rotatebox{70}{Non-exist (E)} & \rotatebox{70}{Non-exist (NE)} & \rotatebox{70}{Partial Actions} & \rotatebox{70}{Time Order} & \rotatebox{70}{Emotional Context} & \rotatebox{70}{Unusual Activities} \\
\hline
\multicolumn{12}{l}{\textbf{GPT-4o mini}} \\
LLaMA-VID & 0.1843 & 0.3549 & 0.4648 & 0.3589 & 0.2768 & \textbf{0.1002} & \textbf{0.0445} & 0.2111 & 0.1422 & 0.1779 & 0.1885 \\
GPT-4o mini & \textbf{0.2487} & 0.0848 & 0.0974 & 0.2579 & 0.1846 & -0.0455 & -0.1566 & 0.0811 & 0.2350 & 0.0096 & -0.0556 \\
Video-ChatGPT & 0.2356 & 0.3811 & \textbf{0.5651} & 0.3987 & \textbf{0.4177} & \textbf{0.2198} & \textbf{0.1679} & 0.1843 & \textbf{0.3795} & 0.2106 & 0.2336 \\
mPLUG-Owl-Video & 0.1703 & \textbf{0.4530} & 0.5542 & \textbf{0.4777} & 0.3472 & \textbf{0.2198} & 0.0704 & \textbf{0.3321} & 0.2821 & \textbf{0.2474} & \textbf{0.2728} \\
Video-LLaVA & 0.1798 & \textbf{0.4625} & 0.3838 & 0.3342 & 0.4136 & 0.1287 & 0.0192 & 0.2319 & 0.2461 & 0.1832 & 0.1739 \\
\textit{Average} & 0.2037 & 0.3472 & 0.4131 & 0.3655 & 0.3280 & 0.1246 & 0.0291 & 0.2081 & 0.2570 & 0.1657 & 0.1626 \\
\hline
\multicolumn{12}{l}{\textbf{InternVL2}} \\
LLaMA-VID & 0.0276 & \textbf{0.1990} & \textbf{0.1144} & 0.1720 & 0.1121 & \textbf{0.0249} & \textbf{-0.0337} & \textbf{0.0463} & -0.0081 & 0.0913 & 0.0037 \\
GPT-4o mini & \textbf{0.1138} & 0.0430 & 0.0880 & \textbf{0.1825} & 0.0429 & -0.1761 & -0.2416 & \textbf{0.0524} & -0.0211 & -0.1335 & -0.1483 \\
Video-ChatGPT & 0.0860 & 0.1855 & \textbf{0.1511} & 0.1409 & 0.1229 & -0.1583 & -0.0420 & -0.0161 & 0.0362 & 0.0438 & 0.0521 \\
mPLUG-Owl-Video & 0.0185 & \textbf{0.2103} & 0.1124 & 0.1181 & \textbf{0.1440} & -0.0023 & -0.0464 & -0.0150 & \textbf{0.0992} & \textbf{0.1034} & \textbf{0.0708} \\
Video-LLaVA & 0.0622 & 0.2096 & 0.0122 & 0.0205 & 0.1269 & -0.0026 & -0.0459 & -0.0258 & 0.0551 & \textbf{0.1086} & 0.0318 \\
\textit{Average} & 0.0616 & 0.1695 & 0.0956 & 0.1268 & 0.1097 & -0.0629 & -0.0819 & 0.0083 & 0.0323 & 0.0427 & 0.0020 \\
\hline
\end{tabular}
\caption{Agreement scores across various CVRR (Computer Vision and Robotics Research) dimensions}
\label{tab:cvrr_scores}
\end{table}
